LLM-as-a-tutor in EFL Writing Education: Focusing on Evaluation of Student-LLM Interaction

In the context of English as a Foreign Language (EFL) writing education, LLM-as-a-tutor can assist students by providing real-time feedback on their essays. However, challenges arise in assessing LLM-as-a-tutor due to differing standards between educational and general use cases. To bridge this gap, we integrate pedagogical principles to assess student-LLM interaction. First, we explore how LLMs can function as English tutors, providing effective essay feedback tailored to students. Second, we propose three metrics to evaluate LLM-as-a-tutor specifically designed for EFL writing education, emphasizing pedagogical aspects. In this process, EFL experts evaluate the feedback from LLM-as-a-tutor regarding quality and characteristics. On the other hand, EFL learners assess their learning outcomes from interaction with LLM-as-a-tutor. This approach lays the groundwork for developing LLMs-as-a-tutor tailored to the needs of EFL learners, advancing the effectiveness of writing education in this context.

==> latex/texes/outdated_related_work.tex <==
In this section, we describe previous studies in feedback generation and LLM evaluation for education.

\subsection{Feedback Generation for Education}
Recent studies discuss that LLM-generated real-time feedback can help education innovation~\cite{yan-2024-practical, kasneci-2023-ChatGPT, wang-demszky-2023-chatgpt}.
However, LLMs often struggle to generate constructive feedback in the context of education.
Unlike human feedback, which consistently identifies points for improvement, GPT-generated feedback then fails to effectively point out students' weaknesses \cite{behzad-etal-2024-assessing}. 
In this study, we first examine the potential of LLMs to serve as English writing tutors and explore methods for generating more effective feedback for students. 
% , but there is no study on how to use LLMs to generate the feedback and how to evaluate the generated feedback to improve education.
% Since feedback is for students and instructors, it is necessary to consider the pedagogical aspects when generating and evaluating feedback in the context of education. 
% While there are several research that evaluate general LLM responses \cite{zheng-2024-judging, wang-etal-2023-cue, jia-2021-all}, we explore LLM feedback on students' essays in the domain of real-world EFL education.

\subsection{LLM Evaluation for Education}
LLM evaluation for general purposes is mainly focused on assessing the quality of the generated response of the model. 
\citet{wang-etal-2023-cue} and \citet{zheng-2024-judging} evaluate the quality of LLM-generated responses under four criteria (helpfulness, relevance, accuracy, and level of detail) and two criteria (helpfulness and acceptability), respectively.
\citet{chang-2024-survey} also defines six criteria (accuracy, relevance, fluency, transparency, safety, and human alignment) for a comprehensive evaluation of the quality of LLM-generated text.
% 그냥 lm의 response를 단순히 평가하는걸 넘어서서 다양한 고려가 필요하다는 점을 시사
However, as \citet{lee-2023-evaluating} points out, merely evaluating the final output quality is insufficient to fully capture the dynamics of human-LM interactions.

% In particular, a more nuanced approach is required to assess educational feedback effectively. 
In AI-integrated education, the evaluation metrics used tend to mirror those applied in broader LLM evaluations. 
Despite this need, existing research often relies on traditional evaluation metrics, which may overlook the complexities of educational settings.
% In the realm of AI-integrated education, the evaluation metrics used tend to mirror those applied in broader LLM evaluations. 
Common human evaluation metrics in education include accuracy \cite{kwon-etal-2024-biped, ross-andreas-2024-toward, luo-etal-2024-chain}, correctness \cite{ross-andreas-2024-toward}, and readability \cite{dai-2023-can}.
% For instance, \citet{dai-2023-can} assesses ChatGPT-generated feedback primarily using two metrics: readability and polarity. 
However, educational feedback requires a more nuanced consideration of factors outside traditional metrics.
Our work incorporates metrics that specifically consider pedagogical factors, going beyond traditional evaluation methods.

In addition, evaluating the learning process and outcomes is challenging and requires the expertise of education professionals. Despite this, many studies rely on human annotators who lack specific expertise in English education \cite{ross-andreas-2024-toward, kwon-etal-2024-biped, luo-etal-2024-chain, jurenka-2024-towards}. In contrast, we involve real-world education stakeholders to better assess human-LM interaction. 


